A Molecular Hyper-message Passing Network with Functional Group Information

We proposed the molecular hyper-message passing network (MolHMPN) that predicts the properties of a molecule with prior knowledge-guided subgraph. Modeling higher-order connectivities in molecules is necessary as changes in both the pair-wise and higher-order interactions among atoms results in the change of molecular properties. Many approaches have attempted to model the higher-order connectivities. However, those methods relied heavily on data-driven approaches, and it is difficult to determine if the utilized subgraphs contain any properties of interest or have any significance on the molecular properties. Hence, we propose MolHMPN to utilize the functional group prior knowledge and model the pair-wise and higher-order connectivities among the atoms in a molecule. Molecules can contain many types of functional groups, which affect the properties the molecules. For example, the toxicity of a molecule is associated with toxicophores, such as nitroaromatic groups and thiourea. MolHMPN uses functional groups to construct hypergraphs, modifies the hypergraph using domain knowledge-guided modification scheme, embeds the graph and hypergraph inputs using a hypergraph message passing (HyperMP) layer, and uses the updated graph and hypergraph embeddings to predict the properties of the molecules. Our model provides a way to utilize prior knowledge in chemistry for molecular properties prediction tasks, and balance between the usage of prior knowledge and data-driven modification adaptively. We show that our model is able to outperform the other baseline methods for most of the dataset, and show that using domain knowledge-guided data-learning iseffective.

==> molhgcn.tex <==
\usepackage[square,numbers]{natbib}
\bibliographystyle{abbrvnat}

==> packages.tex <==
\usepackage{iclr2022_conference,times}
% \usepackage[square,numbers]{natbib}


\input{math_commands.tex}
\definecolor{lightblue}{RGB}{31,119,180}
\definecolor{navy}{RGB}{0,0,128}
\usepackage[colorlinks=true,
            linkcolor=navy,
            citecolor=navy,
            urlcolor=blue]{hyperref}
\usepackage{graphicx}

% Adjust margins for bullet points
\usepackage{enumitem} 

% Table
\usepackage{booktabs}
% \usepackage{multirow}

% Put figures side by side
\usepackage{caption}
\usepackage{subcaption}

% Color dot
\usepackage{tikz}
\usetikzlibrary{shapes}
\usetikzlibrary{plotmarks}

% Colors
\definecolor{repr}{RGB}{255,127,14}
\definecolor{sub}{RGB}{44,160,44}
\definecolor{mult}{RGB}{214,39,40}
\definecolor{molhgcn}{RGB}{31,119,180}

% Green checkmark
\usepackage{xcolor,pifont}
\newcommand*\colourcheck[1]{%
  \expandafter\newcommand\csname #1check\endcsname{\textcolor{#1}{\ding{52}}}%
}

% Adjust margins for bullet points
\usepackage{enumitem} 

\colourcheck{sub}
\newcommand{\xmark}{\ding{55}}%

% subfigures
% \usepackage[caption=false]{subfig}

==> sections/datasets.tex <==
\subsection{Datasets}

\textbf{Tox21} The Toxicology in the 21st Century (Tox21) \cite{molnet:2018, tox21:2015} dataset was created to assess the potential of drugs to disrupt biological pathways that may result in toxicity. It contains 8014 compounds with 12 different targets, which include the nuclear receptor (NR) and stress response (SR) pathways. NRs are one of the essential classes of transcriptional factors that play a critical role in human development, metabolism and physiology. The inappropriate activation of NRs can lead to a broad spectrum of negative health effects. %The NRs that are evaluated includes the estrogen receptor (ER) and its ligand binding domain (ER-LBD), androgen receptor (AR) and its ligand binding domain (AR-LBD), aromatase enzyme (Aromatase), aryl hydrocarbon receptor (AhR), and peroxisome proliferator-activated receptor gamma (PPAR-gamma). 
SR pathways are the cellular and organismal mechanisms that resist the effects of cellular stress, which can lead to apoptosis. 
%The SRs that are evaluated includes the antioxidant response element (ARE), heat shock factor response element (HSE), ATAD5 signaling pathway (ATAD5), mitochondrial membrane potential (MMP), and p53 signaling pathways (P53).

\textbf{ClinTox} The ClinTox dataset compares the drugs that are approved by the FDA and drugs that have failed the clinical tests \cite{molnet:2018}. It contains 1491 drug compounds with 2 tasks: the clinical trial toxicity and the FDA approcal status. 

\textbf{SIDER} The Side Effect Resource (SIDER) \cite{sider} dataset contains information on marketed medicines and their adverse drug reactions. It contains 1427 approved drugs with 27 tasks that are grouped based on their side effects on 27 system organ classes following the MedDRA classifications \cite{meddra}.  

\textbf{BBBP} The Blood-brain barrier penetration (BBBP) dataset was created to model and predict the barrier permeability. The Blood-Brain Barrier separates the circulating blood and the brain extracellular fluid, and protects the brain from foreign substances in the blood that may damage the brain. Hence, BBBP is one of the key factors in chemical toxicological studies and in drug design. The BBBP dataset contains over 2000 compounds with 1 task that evaluates the permeability of the compounds.

\textbf{BACE} The Beta-Secretase 1 (BACE) dataset consists of small molecule inhibitors, and provides quantitative IC50 and qualitative binding results for a set of inhibitors of human beta-secretase 1 (BACE1). BACE is essential for the production of the toxic amyloid beta that is critical in early part in the Alzheimer's disease pathogenesis. The BACE dataset contains 1522 compounds with 1 task that provides the binding results for the inhibitors. 

\textbf{ESOL} The Estimated Solubility (ESOL) dataset contains information on the water solubility of compounds. The knowledge of thermodynamic solubility of drug candidates is important in drug discover as it is related to the drug absorption in the body \cite{soluble:1997}. The ESOL dataset has 1128 compounds.
%https://pubs.acs.org/doi/pdf/10.1021/cc9800071

\textbf{FreeSolv} The Free Solvation Database(FreeSolv) provides the calculated hydration free energy of fragment-like compounds in the water and provides a test of potential relevance to the binding affinity calculations for drug discovery \cite{molnet:2018}. FreeSolv contains 643 compounds. CITATION FREE ENERGY RANGE

%citation for your freesolv bs https://onlinelibrary.wiley.com/doi/epdf/10.1002/minf.201501035

\textbf{Lipophilicity} The Lipophilicity dataset \cite{molkit:2021} was used for the prediction of octanol/water distribution coefficient (logD at pH 7.4). The lipophilicity of drug molecules affects both the membrane permeability and solubility. The Lipophilicity dataset contain 4200 compounds. 

%https://reader.elsevier.com/reader/sd/pii/S0928098715002043?token=481E0F7C9C375DA53527EB2467F2420BAA69C8D3961469E6C974C836736269485C4EA9740D48518D7096A0ADB2C0C90A&originRegion=us-east-1&originCreation=20211201092131

\subsection{Evaluation methods}
\textbf{AUROC} The area under the receiver operating curve (AUROC) is used to evaluate the performances of the classification tasks. 

\textbf{RMSE} The root-mean-square error (RMSE) is used to evaluate the performances of the regression tasks. 
